A Formalism of DNN Accelerator Flexibility

The high efficiency of domain-specific hardware accelerators for machine learning (ML) has come from specialization, with the trade-off of less configurability/ flexibility. There is growing interest in developing flexible ML accelerators to make them future-proof to the rapid evolution of Deep Neural Networks (DNNs). However, the notion of accelerator flexibility has always been used in an informal manner, restricting computer architects from conducting systematic apples-to-apples design-space exploration (DSE) across trillions of choices. In this work, we formally define accelerator flexibility and show how it can be integrated for DSE. Specifically, we capture DNN accelerator flexibility across four axes: tiling, ordering, parallelization, and array shape. We categorize existing accelerators into 16 classes based on their axes of flexibility support, and define a precise quantification of the degree of flexibility of an accelerator across each axis. We leverage these to develop a novel flexibility-aware DSE framework. We demonstrate how this can be used to perform first-of-their-kind evaluations, including an isolation study to identify the individual impact of the flexibility axes. We demonstrate that adding flexibility features to a hypothetical DNN accelerator designed in 2014 improves runtime on future (i.e., present-day) DNNs by 11.8x geomean.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> packages.tex <==
% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{booktabs} % for professional tables
\usepackage{mathtools}
\usepackage{comment}
% \usepackage{epsfig}
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{helvet}  %Required
% \usepackage{courier}  %Required
% \usepackage{url}  %Required
% \usepackage{xcolor}
% \usepackage{multirow}
% \usepackage{subcaption}
% \usepackage{array}
\usepackage{algorithm}
% \usepackage{algorithmic}
% \usepackage{fullpage}
% \usepackage{times}
% \usepackage{xcolor}
% \usepackage{listings}
% \usepackage{titlesec}
% \usepackage[table,xcdraw]{xcolor}
% \usepackage{multirow}
\usepackage{cite}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithmic}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{xspace}
%\usepackage{fancyhdr}
%\usepackage[hyphens]{url}
\usepackage{hyperref}
\usepackage{caption}
\usepackage{ragged2e}
\usepackage{makecell}
\usepackage{tabularx}




==> sections/00_Abstract-old.tex <==
%%% Budget
% Abstract - 0.25 (0.25)
% Intro - 1 (0.75)
% Background - 0.5 (0.75)
% Components of Flexibility - 2 (1.75)
% Flexion - 2 (2.25)
% Methodology - 1 (0.5)
% Case Studies - 4 (4.75-5)
% Related Work - 0.5 (0.5)
% Conclusion - 0.25 (0.25)
% Total = 11

% Candidates to shrink
% MobileNet - one row + shrink text
% Sec V-D -- shrink. One paragraph..
% Sec V-E -- shrink.
% Table II --> remove
% Add a Takeaways paragraph


\begin{abstract}
\TODO{needs to be updated}
Dataflow and tile size choices, which we collectively refer to as mappings, dictate the efficiency (i.e., latency and energy) of DNN accelerators.
%
Rapidly evolving DNN models is one of the major challenges for DNN accelerators since the 
optimal mapping heavily depends on the layer shape and size.
%Since the optimal mapping changes as the layer operation and sizes in DNN models change, .
%
To maintain high efficiency across multiple 
DNN models, 
flexible 
accelerators that can support multiple mapping have emerged.
%maintain high efficiency of DNN accelerators for evolving DNN models, flexible accelerators that support multiple mapping have emerged.
However, the notion of accelerator flexibility has always been used in an informal and qualitative manner.
%Although many flexible accelerators are proposed, 
We currently lack a 
metric to evaluate 
accelerator flexibility 
and quantitatively compare their capability to run different mappings.
%
In this work, 
we formally define the
concept of flexibility in DNN accelerators 
as a quadruple comprising the
supported tile sizes, loop orders, 
parallelism dimensions and array 
shape.
Furthermore, we 
propose \emph{flexion} (\underline{flex}ibility fract\underline{ion}), which is a first-of-its-kind 
quantitative metric of flexibility 
in DNN accelerators.
We also develop a flexibility-aware DSE framework.
%
%
%\TODO{update the takeaways in abstract and intro}
Using these tools, we evaluate the impact of each component of flexibility on accelerator performance, energy, and area through several map-space sweeps. We also perform a case study on future-proofing to identify how an 
accelerator designed for Alexnet in 2014 with varying degrees of flexibility would perform on 
models in use today.
%
%\TODO{update:
%We show that Eyeriss-like accelerator is \rev{2.2$\times$} and \rev{17.0$\times$} more flexible (i.e., capable of running more mappings) than NVDLA and TPUv1-based accelerators on selected ResNet-50 \rev{and MobileNetV2} layers.}
% Our study shows that flexibility features related to tile size are significantly more impactful than other classes. Specifically, they demonstrate improvements of \TFlex in flexion, \TPerf in performance, and \TEnergy in energy, while costing only \TArea area overhead. In contrast, features related to array shape improve performance \SPerf and energy \SEnergy, but only increase flexion by \SFlex.
%
%This work is the first work to formalize accelerator flexibility and enable quantitatively compare accelerator flexibillity.

\begin{comment}
%
Because layers in DNN models prefer different dataflow styles and tile sizes, and DNN models evolve fast, many flexible DNN accelerator architectures and tile size optimizers are proposed to provide adaptivity to new DNN models.
%
Although such works presented promising efficiency benefits over costs, we currently lack a methodology to compare the amount of flexibility provided by various accelerator architectures and identify the right amount of flexibility to maximize the benefits over costs.
%
To develop such a methodology, we need to quantify the amount of mapping flexibility and formalize the relationship between the flexibility and hardware component choices (i.e., buffer, NoC, etc.) in accelerators.


Therefore, we first formally define a metric for mapping flexibility, which ranges from 0 (fixed) to 1 (fully flexible), and formalize the impact of hardware component choices on the amount of flexibility.
%
We codify the formalism into a framework, FlexiS, which receives accelerator hardware specification and target DNN model as inputs and reports the flexibility enabled by the accelerator with the estimated latency and energy.
%
We implement a unified design space exploration framework for flexible DNN accelerator architectures upon FlexiS and perform case studies that analyze the hardware costs for flexibility and benefits from the enabled flexibility on five DNN models.
%
We identify the amount of flexibility for evaluated DNN models to maximize benefits is relatively low, 0.13 in our proposed flexibility metric, on average.
%
The results show that flexible accelerator architectures we evaluate provide 3.2X more mapping flexibility than needed to maximize benefits, on average.
\end{comment}


\end{abstract}

==> sections/01_Introduction-old.tex <==
\section{Introduction}
\label{sec:introduction}

\TK{needs to be re-written. I'll add some pointers on flow of intro later this weekend}

% Domain-specific accelerators exhibit significantly increased efficiency for their target workloads, but are not Turing Complete.
% However, many accelerators do retain a degree of configurability, especially related to \emph{data orchestration}: namely, the choices of scheduling data movement, tile size, buffer allocation, and computation ordering. 
% We term the degree of data orchestration configurability as accelerator \emph{flexibility} and distinguish it from the degree of reconfigurability based on functionality (i.e., FPGAs).

%Flexibility is particularly important for deep-learning accelerators, as different deep neural network (DNN) layers can vary significantly in size and shape.
\hl{\textit{Flexibility}, which we define in this work as the ability of a deep neural network (DNN) accelerator to exploit more than one way of running DNN layers, is particularly important for deep-learning %
as different DNN layers can vary significantly in size and shape.}
%accelerators, as different deep neural network (DNN) layers can vary significantly in size and shape.
%
Relying on a single problem dimension (e.g., rows of weights, output channels, etc.) for parallelism or data reuse (\hl{as several inflexible accelerators with hardcoded dataflows do}) can result in significant under-utilization when the dimension is too small.
For example, the CONV2\_1 early layer in ResNet-50 has 56x56 activations with 64 channels, whereas the CONV5\_3 late layer in ResNet-50  has 7x7 activations with 2048 channels.
A mapping that exploits parallelism on activations can result in severe underutilization on the late layer, and vice versa for one that exploits parallelism on channels.
%MobileNetv2~\cite{sandler2018mobilenetv2} the ratio of activation width to channels reaches 1280, but in ResNet-50~\cite{he2016deep} it is 292.57.
There is extensive evidence that the optimal \hl{dataflow} can vary both across and within networks \cite{kwon2020maestro, parashar2019timeloop}.

% commented for MICRO 2021 revision
%data orchestration configuration can vary both across and within networks \cite{kwon2020maestro, parashar2019timeloop}.

%Collectively, these are called an accelerator's \emph{dataflow}. TODO: history of dataflow here from Eyeriss through TimeLoop, introduce term mapping. In this paper we use the term \emph{flexibility} to refer to an accelerator's ability to adapt its mapping towards an optimal execution of its input data.


%This concept of flexibility is particularly important in the field of deep learning accelerators; different neural network layer sizes can significantly differ in data shapes and ratios, and often  prefer different scheduling strategies. 
%For example, if an accelerator tries to exploit parallelism=64 across input channels, than a network like MobileNet which only has 16 channels will result in under-utilization. 
%On the other hand, an accelerator that exploits parallelism=64 across activation height would find itself under-utilized on 49 of Resnet50's 50 layers.
%An architecture that was flexible enough to perform either mapping would not be under-utilized in either case.

%\input{tables/area_power_latency.tex}

Furthermore, the field of DNNs is changing rapidly, with new networks being proposed at a breakneck pace.
Architects cannot see the future and so must make decisions today based on finite benchmark sets and a limited ability to predict trends in neural networks, knowing that it may be several years before their design reaches the field.
From this point of view, flexibility is desirable for ``future-proofing'' as well, but whether or not this investment pays off can only be quantified post-facto.

This leads to an intractable 
conundrum.
% commented for MICRO 2021 revision
%computer architecture problem. 
%that we term the \textit{Accelerator Mapping Flexibility Conundrum}. 
Namely, investing in hardware features for flexibility consumes resources that could be applied elsewhere---most notably area and energy, but also significant engineering effort in design/verification of the reconfiguration toolchain. 
Therefore, even if a strong predictive case can be made for flexibility features, they often end up ``on the cutting room floor'' when faced with real-world budgeting of area/energy/effort.

%\TK{might be good to point to the TPU as an example for this which is inflexible and uses the area to just scale-up an inflexible array}

In order to break this conundrum,
this paper makes three key contributions to the field of domain-specific accelerators.
%\HK{I couldn't get what the next sentence means. Immediate questions comes into my mind are as follows: (1) What are those four components? (2) Why 16 classes? Is each component binary so we got 16? (3) What is Flexibility TOPS?}
%\HK{ I also suggest to change "First," "Second," "Third" to a more explicit way such as: }

\textbf{Contribution 1:} We identify and 
formally define four components of flexibility---tile size (T), order (O), parallelism (P) and array shape (S), which we term as Flexibility TOPS (as an analog to Performance TOPS \cite{tops_definition}).
%\angshu{any reason why Order is capitalized?}
Identifying each component with a binary 0/1 value
enables us to create 
16 flexibility classes within which 
various accelerators can fall. 
This contribution paves the way for 
a systematic study 
of the specific hardware features needed for implementing each component of flexibility.
%that an architect may wish to invest in and study the cost-benefit trade-off.

\textbf{Contribution 2:} We propose a first-of-its-kind quantitative metric of accelerator flexibility called \emph{flexibility fraction} or \emph{flexion}\footnote{Pronounced ``fleck-shun.'' In biology this term refers to the act of bending a joint or limb, so we find it particularly suitable for a flexibility metric.} defined as
% In contrast with Turing Completeness, our goal is not binary yes/no judgement, but rather a \emph{flexibility fraction} or \emph{flexion}\footnote{Pronounced ``fleck-shun.'' In biology this term refers to the act of bending a joint or limb, so we find it particularly suitable for a flexibility metric.} of the general form:
\[
\frac{Mappings_{supported}}{Mappings_{possible}}
\]
\noindent Where $Mappings_{possible}$ is all possible mappings for the network layer being mapped on a fully flexible accelerator,
and $Mappings_{supported}$ is the number of those mappings that the specific measured accelerator can exploit.  
%The \flexion reflects the ratio of exploitable mapping space to the entire mapping space (with some restrictions to avoid infinity that we detail).
%
%\begin{itemize}
%    \item $Mappings_{Possible}$ derives only from the network layer being mapped, and is the same across all accelerators (with some key restrictions to avoid infinity that we detail), and
%    \item $Mappings_{Supported}$ is the number of those mappings that the specific accelerator design being measured can exploit.
%\end{itemize} 
%
In the limit a fully-fixed accelerator should approach 0 and a fully-flexible accelerator should approach 1.
However this depends on the amount of 
intersection between 
an accelerator's configuration-space and a workload's 
map-space as we discuss.
Additionally, keeping the numerator and denominator separate clarifies apples-to-apples comparisons, such as during design-space exploration (DSE).
%Ultimately, we hope that our metric can be paired with well-understood area/energy quantification techniques to create a comprehensive flexibility cost/benefit analysis of buffering, control, and network-on-chip hardware features.


% \textbf{Contribution 3:}We pair our proposed metric with well-understood performance, area, and energy quantification techniques to create a first-of-its-kind study of the performance versus cost (area and/or power due to buffering, control, and network-on-chip hardware features) across degrees of flexibility. Our study shows that the tile size (T) class of features is significantly more impactful than the others. Specifically, it demonstrates improvements of \TFlex in flexibility, \TPerf in performance, and \TEnergy in energy, while costing only \TArea area overhead. This leads us to recommend these specific features as the most impactful for architects looking to ``future-proof'' their designs. In contrast, features related to array shape improve performance \SPerf and energy \SEnergy, but only increase flexion by \SFlex, and thus are more suitable for designs whose workloads are expected to remain stable after deployment.


\textbf{Contribution 3:} We pair our proposed metric with well-understood performance, area, and energy quantification techniques to create a first-of-its-kind flexibility-aware DSE framework to study %of 
the performance versus cost (area and/or power due to buffering, control, and network-on-chip hardware features) across the four components of
of flexibility. 
Flexion complements enables a more precise quantitative comparison across potential design points of the same accelerator and also %comparison 
across accelerators.
%Our flexibility metrics and our evaluation framework is generic and are capable of evaluating arbitrary DNN layers and models (and even other applications beyond neural networks). In this work,
We showcase the approach by evaluating popular DNN applications with widely varying characteristics: vision, language, and recommendation models through several case studies.

%\TODO{update the takeaways}

%\textbf{Relevance of flexibility in design-space explorations.}
\textbf{Key Takeaways.}
Fundamentally, the value of ``future-proofing'' an accelerator can only be quantified post-facto. 
%However, our approach demonstrates that including flexibility as an optimization criteria in architectural exploration phase can lead to novel key insights that may be otherwise overlooked.
\hl{However, we gain novel insights into its value by examining how a flexible accelerator designed for Alexnet} \cite{alexnet} \hl{circa 2014 would have performed on networks released subsequently, if it had been designed with high and low flexion.}
Specifically:
\squishlist
% Commenting out for MICRO 2021 revision
%\item Our studies shows that the area cost of each class of feature from low to high is: Tile (T), Shape (S), Parallelism (P) and Order (O).
%%Independently, (T) and (P) yield the most performance gain and (S) the least.

\item \hl{Area overheads for flexibility are low (+0.37\%) in practice. The energy overheads pay for itself via more efficient mappings.}

\item \hl{Flexibility can significantly improve runtime on the future networks (11.8$\times$ geo. mean).}

\item {For Mnasnet, independently, (T) and (P) yield the most (4.8x/1.7x) performance gain and (S) the least (1.04x)}.
%
%\item \hl{(P)+(S) together gain huge performance jump over independent (P) or (S).}
% \item The gain from (S) is highly tied to (P) and vice versa.

\item \hl{``Partially'' flexible accelerators -- easier to build and program -- can sometimes provide similar benefits to fully-flexible ones (12-57\% depending on the network).}

% \item Smaller-sized accelerators gain more value from flexibility than larger counterparts since the set of mappings they can run are already quite restricted by the size of the array and buffers.

\item \hl{For models formed with similar set of layers, (T) offered the most valuable flexibility (3.2x speedup). For diverse models, investing in (P) and (S) together offered higher benefits in runtime (49\%) compared to investing in only one of them (8-18\%).}

% \item To future-proof against the same class of models, we find flexibility in (T) is most valuable. For future-proofing against diverse layer types, investing in (P)+(S) is crucial.

\squishend

\hl{In all, we hope that quantifying the benefits of flexibility can help the community better understand the value of investing engineering effort into flexible hardware and the software toolchains required to exploit it.}

%Across multiple interacting classes, we find (O)+(T) and (O)+(P) yield the most performance boost, while additionally being the most area-efficient combinations.
%Thus we conclude that flexible buffering schemes and address generation FSMs offer engineering teams the highest return-on-investment of contemporary flexibility features.




% The framework allows us to recommend different flexibility class for architects working with different HW budget and DNN applications, and looking to ``future-proof'' their designs}

% Our study shows that the tile size (T) class of features is significantly more impactful than the others. Specifically, it demonstrates improvements of \TFlex in flexibility, \TPerf in performance, and \TEnergy in energy, while costing only \TArea area overhead. This leads us to recommend these specific features as the most impactful for architects looking to ``future-proof'' their designs. In contrast, features related to array shape improve performance \SPerf and energy \SEnergy, but only increase flexion by \SFlex, and thus are more suitable for designs whose workloads are expected to remain stable after deployment.

%\textcolor{red}{\textbf{Value of formalizing flexibility for design-space exploration.} DSE
%for DNN accelerators today optimizes the hardware (including dataflow and compute-memory resources) and mappings for a set of target DNN models. The aim of this work is to enable 
% DSE for  ``future-proofing". 
%To this end, identifying four specific hardware features 
%for enabling flexibility (namely tile sizes, computation order, parallelism, and array shape via Contribution 1) can enable architects 
%to systematically study 
%trade-offs between the accelerator's coverage of the mapping space (quantified as flexion via Contribution 2), performance benefits, and cost
%(quantified through our flexibility-aware DSE framework via Contribution 3).
%}

% Tushar: Commented out Felix's  text:
%We formalize the flexibility of an accelerator by categorizing it into one of the 16 \textbf{\textit{flexibility classes}}, implying its ability to explore different dimensions of DNNs mapping, and a \textbf{\textit{flexion score}}, which quantify this flexibility by the ratio of number of available-to-explore mapping to the entire mapping space.
%The formalization allows us i) to explicitly show the change of the available mapping space (\textit{flexion}) while adding different HW components into accelerators, and ii) to recommend different flexibility feature (\textit{flexibility classes}) for architects working with different HW budget and DNN applications and looking to ``future-proof'' their designs in a systematic manner. }

%Ultimately, we hope that the ability to quantify flexibility will open up notable avenues of future research, leveraging the traditional quantitative approaches of computer architecture tradeoffs and DSE to solve the conundrum of flexibility.

% Ultimately, our metric can be paired with well-understood area/energy quantification techniques to create a comprehensive flexibility cost/benefit analysis of buffering, control, and network-on-chip hardware features, as an example in~\autoref{tab:trade_off_study_example}.

%\HK{Since we already discussed the contributions, briefly summarizing the future impact of this work (i.e., Solving Mapping Flexibility Conundrum) with the key results might be a good idea.}

\begin{comment}
This paper offers the following specific contributions:

\begin{itemize}
    \item A formal, quantified metric for flexibility, including a discussion of how the metric deals with potentially-infinite design spaces.
    \item A quantitative evaluation that applies the metric to specific accelerator features, including buffering and network-on-chips, and characterizes their impact on overall accelerator flexibility.
    \item A quantification of several existing deep learning accelerators according to the metric.
\end{itemize}

Finally, we pose a new problem statement which we term the Strong Accelerator Flexibility Hypothesis. This serves as a sort of ``grand challenge'' of future work to the domain-specific accelerator community that answers that value of flexibility features finally and definitively.



%Although all of such works presented promising results with reconfigurable accelerators, we currently lack a unified methodology to compare the degree of flexiblity each design provides.
%
%Therefore, in this chapter, we propose a metric of mapping flexiblity in DNN accelerators, and clarify how the choice of hardware components constraint possible mappings on DNN accelerators.
%

%List of contributions:
%\squishlist
%{\item Formalization of the problem}
%{\item Quantification of the problem}
%{\item Actual analysis in case studies}
%\squishend

%<Naming the problem?>
%Gordian Knot?
%Paradox (X)
%Flexibility Conundrum - Invest engineering effort, etc. - will it pay-off?
%Confounding
%Flexibility Hypothesis

%Programmability - functionality 

\end{comment}


==> sections/Note_revision.tex <==
These are the cut down for the revision. We can consider to put them back in the next version.
1. I cut the fig 8 into one column.
2. I takeout the early-layer figure and explanation of Mbnet-L1.


==> tables/area_power_latency.tex <==
\begin{table}[]
\centering
\caption{\rev{An example trade-off study of 256-PE-Eyeriss-, NVDLA-, and TPU-like accelerators (EL, NL, and TL) implemented in RTL and synthesized using 28nm library. We run MAESTRO~\cite{kwon2020maestro} with optimized mapping generated by GAMMA~\cite{shengchun2020gamma} to estimate the latency. We quantify the flexibility of each accelerator Flexion. RC layers are from Resnet50~\cite{he2016deep}, and MB layers are from MobileNetV2~\cite{sandler2018mobilenetv2} as listed in~\autoref{sec:case_study}.}
\vspace{-3mm}}
\label{tab:trade_off_study_example}
\footnotesize
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{\rev{Acc.}}
& \textbf{\rev{Area($mm^2$})}
& \textbf{\rev{Power($mW$)}}
& \textbf{\rev{Layer}}
& \textbf{\rev{Latency}}
& \textbf{\rev{Flexion}} \\
\hline
\multirow{7}{*}{\rev{EL}}
    & \multirow{7}{*}{\rev{5.13}}
        & \multirow{7}{*}{\rev{188.33}} 
            & \rev{RC2\_3}
            & \rev{4.92E+03}
            & \rev{2.23E-04} \\
            \cline{4-6}
            &
            &
            & \rev{RC3\_2}
            & \rev{2.02E+04}
            & \rev{7.53E-05} \\
            \cline{4-6}
            & 
            &
            & \rev{RC5\_2}
            & \rev{3.27E+04}
            & \rev{1.57E-05} \\
            \cline{4-6}
            & 
            &
            & \rev{MB1\_DW}
            & \rev{4.17E+03}
            & \rev{4.15E-06} \\
            \cline{4-6}
            & 
            &
            & \rev{MB5\_DW}
            & \rev{1.14E+03}
            & \rev{4.57E-06} \\
            \cline{4-6}
            & 
            &
            & \rev{MB6\_R}
            & \rev{2.34E+02}
            & \rev{2.33E-03} \\
            \cline{4-6}            
            & 
            &
            & \rev{Avg.}
            & \rev{1.06E+04}
            & \rev{4.77E-05} \\
            \cline{4-6}            
\hline
\multirow{7}{*}{\rev{NL}}
    & \multirow{7}{*}{\rev{3.85}}
        & \multirow{7}{*}{\rev{100.18}} 
            & \rev{RC2\_3}
            & \rev{1.39E+05}
            & \rev{6.24E-07} \\
            \cline{4-6}
            &
            &
            & \rev{RC3\_2}
            & \rev{3.96E+04}
            & \rev{5.29E-06} \\
            \cline{4-6}
            & 
            &
            & \rev{RC5\_2}
            & \rev{8.43E+03}
            & \rev{1.10E-05} \\
            \cline{4-6}
            & 
            &
            & \rev{MB1\_DW}
            & \rev{5.11E+03}
            & \rev{7.69E-08} \\
            \cline{4-6}
            & 
            &
            & \rev{MB5\_DW}
            & \rev{4.02E+03}
            & \rev{2.90E-06} \\
            \cline{4-6}
            & 
            &
            & \rev{MB6\_R}
            & \rev{1.26E+03}
            & \rev{7.71E-03} \\
            \cline{4-6}
            & 
            &
            & \rev{Avg.}
            & \rev{3.29E+04}
            & \rev{6.30E-06} \\
            \cline{4-6}                
\hline
\multirow{7}{*}{\rev{TL}}
    & \multirow{7}{*}{\rev{1.82}}
        & \multirow{7}{*}{\rev{40.79}} 
            & \rev{RC2\_3}
            & \rev{5.67E+04}
            & \rev{1.73E-08} \\
            \cline{4-6}
            &
            &
            & \rev{RC3\_2}
            & \rev{6.79E+04}
            & \rev{1.49E-07} \\
            \cline{4-6}
            & 
            &
            & \rev{RC5\_2}
            & \rev{1.25E+04}
            & \rev{3.11E-07} \\
            \cline{4-6}
            & 
            &
            & \rev{MB1\_DW}
            & \rev{5.08E+03}
            & \rev{7.69E-08} \\
            \cline{4-6}
            & 
            &
            & \rev{MB5\_DW}
            & \rev{1.94E+03}
            & \rev{2.90E-06} \\
            \cline{4-6}
            & 
            &
            & \rev{MB6\_R}
            & \rev{3.29E+02}
            & \rev{7.71E-03} \\
            \cline{4-6}           
            & 
            &
            & \rev{Avg.}
            & \rev{2.41E+04}
            & \rev{1.05E-06} \\
            \cline{4-6}             
\hline
\end{tabular}
\end{table}

==> tables/eval_accelerators.tex <==
\begin{table}[]
\centering
\caption{A list of evaluated accelerators based on Eyeriss~\cite{chen2016eyeriss}, NVDLA~\cite{nvdla}, and TPUv1~\cite{jouppi2017datacenter}. SF, RF, AT, and Spad refer to store-and-forward, reduce-and-forward, adder tree, and scratchpad.\TK{not referred to right now. Either refer to it for Fig 7 or remove it}\vspace{-2mm}}
\label{tab:eval_accelerators}
\footnotesize
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Accelerator}
& \textbf{D. NoC (L2/L1)}
& \textbf{R. NoC (L2/L1)}
& \textbf{Buffer (L2/L1)} \\
\hline
Eyeriss-like
&
Bus / Bus
&
RF / Temporal
&
Spad / Spad \\
\hline
NVDLA-like
&
Bus / Bus
&
Temporal / AT
&
Spad / FIFO \\
\hline
TPUv1-like
&
SF / SF
&
Temporal / RF
&
Spad / FIFO \\
\hline
\end{tabular}
\end{table}

==> tables/flexibility_classes.tex <==
\begin{table}[]
\centering
\caption{Flexibility Classes}
\vspace{-2mm}
\label{table:flexibility_classes}
\footnotesize
\begin{tabularx}{\columnwidth}{|c|c|X|}
\hline
\textbf{} & \textbf{[Tile, Order, Par, Shape]} &  \textbf{Accelerator}\\\hline
Class 0 & [0,0,0,0] & TPUv1~\cite{tpuv1}, ShiDianNao~\cite{du2015shidiannao}  \\\hline
Class 1 & [0,0,0,1] & Eyeriss~\cite{chen2016eyeriss}  \\\hline
Class 2 & [0,0,1,0] &   \\\hline
Class 3 & [0,0,1,1] &   \\\hline
Class 4 & [0,1,0,0] &   \\\hline
Class 5 & [0,1,0,1] &   \\\hline
Class 6 & [0,1,1,0] &   \\\hline
Class 7 & [0,1,1,1] &   \\\hline
Class 8 & [1,0,0,0] &  AI-MT~\cite{aimt}, TPUv3~\cite{cloudtpu} SIMBA~\cite{simba} \\\hline
Class 9 & [1,0,0,1] &  Planaria~\cite{planaria}, Dyhard-DNN~\cite{dyhard_dac2018}, Tangram~\cite{tangram_asplos2019} \\\hline
Class 10 & [1,0,1,0] &   \\\hline
Class 11 & [1,0,1,1] & Eyeriss\_v2~\cite{eyev2}  \\\hline
Class 12 & [1,1,0,0] &  NVDLA~\cite{nvdla} \\\hline
Class 13 & [1,1,0,1] &   \\\hline
Class 14 & [1,1,1,0] &  Flexflow~\cite{lu2017flexflow} \\\hline
Class 15 & [1,1,1,1] & MAERI~\cite{kwon2018maeri}, SIGMA~\cite{qin2020sigma} \\\hline

\end{tabularx}
\end{table}

==> tables/flexibility_components.tex <==
\begin{table}[]
\centering
\caption{Components of Flexibility: T, O, P, and S \TK{can be removed}}
\vspace{-2mm}
\label{table:flexibility_components}
\footnotesize
\begin{tabular}{|c|c|}
\hline
\textbf{Flexibility Component} & \textbf{Hardware Support} \\\hline
Tile Sizes (T) & Soft-partitioned Scratchpads \\\hline
Loop Order (O) & Configurable scratchpad address generators \\\hline
Parallelism Dimension (P) & NoC support for Multicast and Reduction \\\hline
Array Shape (S) & NoC support for PE clustering\\\hline
\end{tabular}
\end{table}

==> tables/flexion_def.tex <==
\begin{table}[]
\centering
\caption{\flexion definition}

\label{table:flexion_def}
\footnotesize


\begin{tabularx}{8.5cm}{|c|X|}
\hline
\textbf{\flexion} & \textbf{Definition} \\\hline
$A_{X}/F_{X}$ & Target accelerator configuration-space flexion (aka hardware flexion). \\\hline
$A^{\omega}_{X}/F^{\omega}_{X}$ & Target accelerator workload relevant configuration-space flexion \\\hline
$F^{\omega}_{X}/W^{\omega}_{X}$ & Resource-constrained fully-flexible accelerator workload-relevant map-space flexion. \\\hline
$A^{\omega}_{X}/W^{\omega}_{X}$ & target accelerator workload-relevant map-space flexion (aka workload flexion). \\\hline
\end{tabularx}

\end{table}




==> tables/layer_by_layer_eval_results.tex <==
\begin{table}[]
\centering
\caption{Tiling (Tl), spatial (Sp), and loop order (Lo) flexibility and resulting flexibility metric. C1,C2,C3, and FC refer to CONV2\_3, CONV3\_2, CONV5\_2, and FC layers in Resnet50~\cite{he2016deep}}
\label{tab:eval_results}
\footnotesize
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Acc.}
& \textbf{Layer}
& \textbf{Tl-Flex.}
& \textbf{Sp-Flex.}
& \textbf{Lo-Flex.}
& \textbf{Flex. Mtrc.} \\
\hline
\multirow{4}{*}{EL-A}
&
C1
&
$8.6 \times 10^{-2}$
&
$2.5 \times 10^{-1}$
&
$2.8 \times 10^{-2}$
&
$6.0 \times 10^{-4}$ \\
\cline{2-6}
&
C2
&
$2.7 \times 10^{-2}$
&
$2.5 \times 10^{-1}$
&
$2.8 \times 10^{-2}$
& 
$1.9 \times 10^{-4}$ \\
\cline{2-6}
&
C3
&
$3.5 \times 10^{-2}$
&
$2.5 \times 10^{-1}$
&
$2.8 \times 10^{-2}$
&
$2.4 \times 10^{-5}$ \\
\cline{2-6}
&
FC
&
$1.3 \times 10^{-5}$
&
$2.5 \times 10^{-1}$
&
$2.8 \times 10^{-2}$
&
$9.0 \times 10^{-8}$ \\
\hline
\end{tabular}
\end{table}

==> tables/scheme_table.tex <==


\begin{table}[t]

\centering
\caption{The 16 categories of TOPS options. }
%\TK{It would be great if in this table, Gene can be defined for what it means in G-SHARP. Similarly, genome uses the word feature which is not defined.}\FK{Fixed.}}

\includegraphics[width=1\linewidth]{figures/scheme_table.pdf}
\vspace{-0.5cm}
\label{table:16categories}
\end{table}


==> tables/space_def.tex <==
\begin{table}[]
\centering
\caption{Terminology.}

\label{table:space_def}
\footnotesize


\begin{tabularx}{8.5cm}{|c|X|}
\hline
\textbf{Term} & \textbf{Definition} \\\hline
$A_{X}$ & Target accelerator supported configuration space. \\\hline
$F_{X}$ & Fully flexible accelerator supported configuration space.\\\hline
$A^{\omega}_{X}$ & $A_{X}$$\cap$$W^{\omega}_{X}$. Target accelerator supported map space for workload $\omega$.\\\hline
$F^{\omega}_{X}$ & $F_{X}$$W^{\omega}_{X}$. Resource-constrained fully-flexible accelerator supported map space for workload $\omega$.\\\hline
$W^{\omega}_{X}$ & Unconstrained-map space for workload $\omega$. \\\hline

\end{tabularx}

\end{table}


==> tables/table_flexbility_classes_ref.tex <==
\nocite{tpuv1,du2015shidiannao,chen2016eyeriss,aimt,cloudtpu,simba,planaria,dyhard_dac2018,tangram_asplos2019,eyev2,nvdla,lu2017flexflow,kwon2018maeri,qin2020sigma}


==> tables/tile_sizes.tex <==
\begin{table*}[]
\centering
\caption{The number of achievable tile size combinations on evaluated Resnet50~\cite{he2016deep} layers (CNV and FC refer to CONV2D and fully-connected layers). The accelerator labels are the same as~\autoref{fig:Flexibility_Metric}. FullFlex refers to a fully-flexible accelerator with infinite size of scratchpad buffers.}
\label{tab:tile_sizes}
\footnotesize
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Acc.}
& \textbf{CNV2\_3}
& \textbf{CNV3\_2}
& \textbf{CNV5\_2}
& \textbf{FC}
& \textbf{B1\_1\_2}
& \textbf{B5\_2\_2}
& \textbf{B6\_R}
& \textbf{Avg.} \\
\hline
EL-A
& 5.6E+12
& 9.1E+10
& 8.8E+09
& 6.1E+09
&
&
&
& 1.4E+12
\\
\hline
EL-B
& 6.8E+11
& 1.2E+09
& 5.9E+07
& 1.0E+08
&
&
&
& 1.7E+11
\\
\hline
EL-C
& 1.5E+13
& 2.3E+11
& 1.4E+10
& 1.4E+07
&
&
&
& 3.8E+12
\\
\hline
NL-A
& 8.7E+08
& 3.6E+08
& 3.4E+08
& 9.0E+08
&
&
&
& 6.2E+08
\\
\hline
NL-B
& 8.4E+08
& 4.3E+07
& 3.3E+07
& 1.0E+08
&
&
&
& 2.5E+08
\\
\hline
NL-C
& 4.8E+08
& 1.9E+08
& 2.7E+08
& 9.0E+08
&
&
&
& 4.6E+08
\\
\hline
TL-A
& 8.7E+08
& 3.6E+08
& 3.5E+08
& 9.2E+08
&
&
&
& 6.2E+08
\\
\hline
TL-B
& 8.4E+08
& 4.3E+07
& 3.3E+07
& 1.0E+08
&
&
&
& 2.5E+08
\\
\hline
TL-C
& 4.8E+08
& 1.9E+08
& 2.7E+08
& 9.2E+08
&
&
&
& 4.7E+08
\\
\hline
FullFlex
& 1.74E+14
& 8.40E+12
& 3.88E+12
& 1.05E+12
&
&
&
& 4.69E+13
\\
\hline
\end{tabular}
\end{table*}
